Parabolic Relaxation for Quadratically-constrained Quadratic Programming -- Part II: Theoretical & Computational Results

In the first part of this work [32], we introduce a convex parabolic relaxation for quadratically-constrained quadratic programs, along with a sequential penalized parabolic relaxation algorithm to recover near-optimal feasible solutions. In this second part, we show that starting from a feasible solution or a near-feasible solution satisfying certain regularity conditions, the sequential penalized parabolic relaxation algorithm convergences to a point which satisfies Karush-Kuhn-Tucker optimality conditions. Next, we present numerical experiments on benchmark non-convex QCQP problems as well as large-scale instances of system identification problem demonstrating the efficiency of the proposed approach.

==> Plot_01.tex <==
\begin{figure}
\captionsetup[subfigure]{position=b}
%\centering
\begin{tikzpicture}[scale=0.7]
\centering
\begin{axis}[
		width = 0.72\textwidth,
		height = 0.42\textwidth,
 		xmode=normal,
		ymode=log,	
    	xlabel={\large$\eta$},
    	ylabel={$\tr\{\Xbf\!-\!\xbf\xbf^{\top}\!\}$},
    	ylabel shift =0cm,
 		xmin=0,
	 	xmax=4,
%         xtickmax = 7500,
%	ymin=1e-5, 
% 	 	ymax= 50,
%   xtick={0,100,200,300,400},
%   ytick={1e-6, 1e-5, 1e-4, 1e-3, 1e-2, 1e-1},
%         xtick scale label code/.code={\pgfmathparse{int(#1)}$\eta \times 10^{-\pgfmathresult}$},
%  		every x tick scale label/.style={at={(xticklabel cs:0.5)}, anchor = north},
% 		scaled x ticks = base 10:-3,
    	legend pos=south west,
    	ymajorgrids=true,
		xmajorgrids=true,
    	grid style=dashed,
	    legend cell align={left},
        legend image post style={scale=0.7},
        legend style={font=\small, inner xsep=0.2pt, inner ysep=0.1pt},
]
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:1.84,0.01)--(axis cs:4,0.01) node [black, pos=0.6, above] {\footnotesize \raisebox{-0.25ex}[0pt][-0.25ex]{$\Xbf\!=\!\xbf\xbf^{\top}$}};
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:2.57,0.001)--(axis cs:4,0.001) node [black, pos=0.52, above] {\footnotesize \raisebox{-0.25ex}[0pt][-0.25ex]{$\Xbf\!=\!\xbf\xbf^{\top}$}};
% \draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:5870.92,0.000473)--(axis cs:7950,0.000473) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.25ex}[0pt][-0.25ex]{$\Xbf\!=\!\xbf\xbf^{\top}$}};
\addplot[color=blue,line width=0.5mm] table[x=X,y=Infs_PRB,col sep=comma] {data_mu.csv};
\addplot[dashed,color=red,line width=0.5mm] table[x=X,y=Infs_PRBC,col sep=comma] {data_mu.csv};
%\addplot[dash dot,color=black,line width=0.5mm] table[x=X,y=Infs,col sep=comma] {data_mu.csv};
% \legend{$\mathrm{SDP}$,$\mathrm{SOCP}$,$\mathrm{Parabolic}$}
% \addplot[dashed, color=red,line width=0.5mm] table[x=X,y=Y2,col sep=comma] {Results/testdataErr.csv};
\legend{Standard coordinates,SDP-induced coordinates}
\end{axis}
%\label{fig:EtaEffect_feasibility_violation}
%\end{tikzpicture}

\hspace{6.0cm}

%\begin{tikzpicture}[scale=0.8]
%\centering
\begin{axis}[
		width = 0.72\textwidth,
		height = 0.42\textwidth,
 		xmode=normal,
%       xmode=log,
		ymode=normal,	
        xlabel={\large$\eta$},
        ylabel={$\bar{q}_0(\xbf,\Xbf)$},
		ylabel shift = 0cm,
 		xmin=0,
  		xmax=4,
%     	ymin = 10.0,
%      	ymax = 11.5,
%         ytickmax = 11.4,,
%         xtickmax = 7500,
%    xtick={0,2000,4000,6000,,8000},
%         xtick scale label code/.code={\pgfmathparse{int(#1)}$\eta \times 10^{-\pgfmathresult}$},
%  		every x tick scale label/.style={at={(xticklabel cs:0.5)}, anchor = north},
% 		scaled x ticks = base 10:-3,
% 		ytick={10.00, 10.25, 10.50, 10.75, 11.00, 11.25, 11.50},
%     	yticklabels={~, 10.25, 10.50, 10.75, 11.00, 11.25, 11.50},
    	legend pos= north west,
    	ymajorgrids=true,
		xmajorgrids=true,
    	grid style=dashed,
		legend cell align={left},
        legend image post style={scale=0.7},
        legend style={font=\small, inner xsep=0.2pt, inner ysep=0.1pt},
]
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:1.84,-6.3)--(axis cs:4,-6.3) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.2ex}[0pt][-0.2ex]{$\Xbf\!=\!\xbf\xbf^{\top}$}};
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:2.57,-6)--(axis cs:4,-6) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.2ex}[0pt][-0.2ex]{~~~~~$\Xbf\!=\!\xbf\xbf^{\top}$}};
\addplot[color=blue,line width=0.5mm] table[x=X,y=Cost_PRB,col sep=comma] {data_mu.csv};
\addplot[dashed,color=red,line width=0.5mm] table[x=X,y=Cost_PRBC,col sep=comma] {data_mu.csv};
%\addplot[dash dot,color=black,line width=0.5mm] table[x=X,y=Cost,col sep=comma] {data_mu.csv};,
\legend{Standard coordinates,SDP-induced coordinates}
\end{axis}
\end{tikzpicture}

\caption{%\small 
	Sensitivity of penalization to the choice of penalty parameter $\eta$. For small choices of $\eta$, penalization fails to provide feasible solutions. The feasibility violation $\tr\{\Xbf-\xbf\xbf^{\!\top}\}$ quickly vanishes for the standard and SDP-induced coordinates at $\eta> 2.57$ and $\eta>1.84$, respectively.}
\label{fig:EtaEffect}
\end{figure}


==> Plot_01_copy.tex <==
\begin{figure}
\captionsetup[subfigure]{position=b}
%\centering
\begin{tikzpicture}[scale=0.7]
\centering
\begin{axis}[
		width = 0.72\textwidth,
		height = 0.42\textwidth,
 		xmode=normal,
		ymode=log,	
    	xlabel={\large$\eta$},
    	ylabel={$\tr\{\Xbf\!-\!\xbf\xbf^{\top}\!\}$},
    	ylabel shift =0cm,
 		xmin=0,
	 	xmax=4,
%         xtickmax = 7500,
%	ymin=1e-5, 
% 	 	ymax= 50,
%   xtick={0,100,200,300,400},
%   ytick={1e-6, 1e-5, 1e-4, 1e-3, 1e-2, 1e-1},
%         xtick scale label code/.code={\pgfmathparse{int(#1)}$\eta \times 10^{-\pgfmathresult}$},
%  		every x tick scale label/.style={at={(xticklabel cs:0.5)}, anchor = north},
% 		scaled x ticks = base 10:-3,
    	legend pos=south west,
    	ymajorgrids=true,
		xmajorgrids=true,
    	grid style=dashed,
	    legend cell align={left},
        legend image post style={scale=0.7},
        legend style={font=\small, inner xsep=0.2pt, inner ysep=0.1pt},
]
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:1.84,0.01)--(axis cs:4,0.01) node [black, pos=0.6, above] {\footnotesize \raisebox{-0.25ex}[0pt][-0.25ex]{$\Xbf\!=\!\xbf\xbf^{\top}$}};
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:2.57,0.001)--(axis cs:4,0.001) node [black, pos=0.52, above] {\footnotesize \raisebox{-0.25ex}[0pt][-0.25ex]{$\Xbf\!=\!\xbf\xbf^{\top}$}};
% \draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:5870.92,0.000473)--(axis cs:7950,0.000473) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.25ex}[0pt][-0.25ex]{$\Xbf\!=\!\xbf\xbf^{\top}$}};
\addplot[color=blue,line width=0.5mm] table[x=X,y=Infs_PRB,col sep=comma] {data_mu.csv};
\addplot[dashed,color=red,line width=0.5mm] table[x=X,y=Infs_PRBC,col sep=comma] {data_mu.csv};
%\addplot[dash dot,color=black,line width=0.5mm] table[x=X,y=Infs,col sep=comma] {data_mu.csv};
% \legend{$\mathrm{SDP}$,$\mathrm{SOCP}$,$\mathrm{Parabolic}$}
% \addplot[dashed, color=red,line width=0.5mm] table[x=X,y=Y2,col sep=comma] {Results/testdataErr.csv};
\legend{Standard coordinates,SDP-induced coordinates}
\end{axis}
%\label{fig:EtaEffect_feasibility_violation}
%\end{tikzpicture}

\hspace{6.0cm}

%\begin{tikzpicture}[scale=0.8]
%\centering
\begin{axis}[
		width = 0.72\textwidth,
		height = 0.42\textwidth,
 		xmode=normal,
%       xmode=log,
		ymode=normal,	
        xlabel={\large$\eta$},
        ylabel={$\bar{q}_0(\xbf,\Xbf)$},
		ylabel shift = 0cm,
 		xmin=0,
  		xmax=4,
%     	ymin = 10.0,
%      	ymax = 11.5,
%         ytickmax = 11.4,,
%         xtickmax = 7500,
%    xtick={0,2000,4000,6000,,8000},
%         xtick scale label code/.code={\pgfmathparse{int(#1)}$\eta \times 10^{-\pgfmathresult}$},
%  		every x tick scale label/.style={at={(xticklabel cs:0.5)}, anchor = north},
% 		scaled x ticks = base 10:-3,
% 		ytick={10.00, 10.25, 10.50, 10.75, 11.00, 11.25, 11.50},
%     	yticklabels={~, 10.25, 10.50, 10.75, 11.00, 11.25, 11.50},
    	legend pos= north west,
    	ymajorgrids=true,
		xmajorgrids=true,
    	grid style=dashed,
		legend cell align={left},
        legend image post style={scale=0.7},
        legend style={font=\small, inner xsep=0.2pt, inner ysep=0.1pt},
]
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:1.84,-6.3)--(axis cs:4,-6.3) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.2ex}[0pt][-0.2ex]{$\Xbf\!=\!\xbf\xbf^{\top}$}};
\draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:2.57,-6)--(axis cs:4,-6) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.2ex}[0pt][-0.2ex]{~~~~~$\Xbf\!=\!\xbf\xbf^{\top}$}};
\addplot[color=blue,line width=0.5mm] table[x=X,y=Cost_PRB,col sep=comma] {data_mu.csv};
\addplot[dashed,color=red,line width=0.5mm] table[x=X,y=Cost_PRBC,col sep=comma] {data_mu.csv};
%\addplot[dash dot,color=black,line width=0.5mm] table[x=X,y=Cost,col sep=comma] {data_mu.csv};,
\legend{Standard coordinates,SDP-induced coordinates}
\end{axis}
\end{tikzpicture}

\caption{%\small 
	Sensitivity of penalization to the choice of penalty parameter $\eta$. For small choices of $\eta$, penalization fails to provide feasible solutions. The feasibility violation $\tr\{\Xbf-\xbf\xbf^{\!\top}\}$ quickly vanishes for the standard and SDP-induced coordinates at $\eta> 2.57$ and $\eta>1.84$, respectively.}
\label{fig:EtaEffect}
\end{figure}

